Proceedings of the 18th International Overture Workshop

This volume contains the papers presented at the 18th International Overture Workshop, held online on 7th December 2020. This event was the latest in a series of workshops around the Vienna Development Method (VDM), the open-source project Overture, and related tools and formalisms. VDM is one of the longest established formal methods for systems development. A lively community of researchers and practitioners has grown up in academia and industry has grown around the modelling languages (VDM-SL, VDM++, VDM-RT, CML) and tools (VDMTools, Overture, Crescendo, Symphony, the INTO-CPS chain, and ViennaTalk). Together, these provide a platform for work on modelling and analysis technology that includes static and dynamic analysis, test generation, execution support, and model checking. This workshop provided updates on the emerging technology of VDM/Overture, including collaboration infrastructure, collaborative modelling and co-simulation for Cyber-Physical Systems.

==> 3-Rask/acronyms.tex <==
\newacronym{ast}{AST}{Abstract Syntax Tree}
\newacronym{ct}{CT}{Combinatorial Testing}
\newacronym{czt}{CZT}{Community Z Tools}
\newacronym{dap}{DAP}{Debug Adapter Protocol}
\newacronym{dbgp}{DBGP}{Common DeBugGer Protocol}
\newacronym{gui}{GUI}{Graphical User Interface}
\newacronym{ide}{IDE}{Integrated Development Environment}
\newacronym{lsp}{LSP}{Language Server Protocol}
\newacronym{poc}{PoC}{Proof of Concept}
\newacronym{pog}{POG}{Proof Obligation Generation}
\newacronym{slsp}{SLSP}{Specification Language Server Protocol}
\newacronym{vdm}{VDM}{Vienna Development Method}
\newacronym{vscode}{VS Code}{Visual Studio Code}


==> 3-Rask/listings/LoC_v1.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|}
\hline
\textbf{Directory/File} & \textbf{Code}                     & \textbf{Comment}                 & \textbf{Blank}                   & \textbf{Total}                    \\ \hline
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                                                                                                        \\ \hline
dap                     & 699                               & 450                              & 186                              & 1335                              \\ \hline
json                    & 551                               & 184                              & 128                              & 863                               \\ \hline
lsp                     & 1242                              & 492                              & 257                              & 1991                              \\ \hline
rpc                     & 177                               & 137                              & 54                               & 368                               \\ \hline
vdmj                    & 1940                              & 429                              & 374                              & 2743                              \\ \hline
workspace               & 1438                              & 123                              & 251                              & 1812                              \\ \hline
\textbf{Sum}            & \textbf{6047}                     & \textbf{1815}                    & \textbf{1250}                    & \textbf{9112}                     \\ \hline
\multicolumn{5}{|c|}{VS Code Extension}                                                                                                                               \\ \hline
extension.ts            & \multicolumn{1}{l|}{150}          & \multicolumn{1}{l|}{30}          & \multicolumn{1}{l|}{34}          & \multicolumn{1}{l|}{214}          \\ \hline
package.json            & \multicolumn{1}{l|}{131}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{132}          \\ \hline
syntax highlight        & \multicolumn{1}{l|}{374}          & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{374}          \\ \hline
\textbf{Sum}            & \multicolumn{1}{l|}{\textbf{655}} & \multicolumn{1}{l|}{\textbf{30}} & \multicolumn{1}{l|}{\textbf{35}} & \multicolumn{1}{l|}{\textbf{720}} \\ \hline
\end{tabular}
\end{table}

==> 3-Rask/listings/LoC_v2.tex <==
\begin{table}[]
\centering
\caption{LoC measures for the files and directories used to support VDM in VS Code\protect\footnotemark{}.}
\label{tab:LoC}
\begin{tabular}{|l|r|r|r|r|llllll}
\cline{1-5} \cline{7-11}
\multicolumn{5}{|c|}{LSP/DAP support for VDMJ}                                               & \multicolumn{1}{l|}{} & \multicolumn{5}{c|}{VS Code Extension}                                                                                                                                                                \\ \cline{1-5} \cline{7-11} 
\textbf{Directory/File} & \textbf{Code} & \textbf{Comment} & \textbf{Blank} & \textbf{Total} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Directory/File}} & \multicolumn{1}{r|}{\textbf{Code}} & \multicolumn{1}{r|}{\textbf{Comment}} & \multicolumn{1}{r|}{\textbf{Blank}} & \multicolumn{1}{r|}{\textbf{Total}} \\ \cline{1-5} \cline{7-11} 
dap                     & 699           & 450              & 186            & 1335           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{extension.ts}            & \multicolumn{1}{l|}{150}           & \multicolumn{1}{l|}{30}               & \multicolumn{1}{l|}{34}             & \multicolumn{1}{l|}{214}            \\ \cline{1-5} \cline{7-11} 
json                    & 551           & 184              & 128            & 863            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{package.json}            & \multicolumn{1}{l|}{131}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{1}              & \multicolumn{1}{l|}{132}            \\ \cline{1-5} \cline{7-11} 
lsp                     & 1242          & 492              & 257            & 1991           & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{syntax highlight}        & \multicolumn{1}{l|}{374}           & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{0}              & \multicolumn{1}{l|}{374}            \\ \cline{1-5} \cline{7-11} 
rpc                     & 177           & 137              & 54             & 368            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Sum}}            & \multicolumn{1}{l|}{\textbf{655}}  & \multicolumn{1}{l|}{\textbf{30}}      & \multicolumn{1}{l|}{\textbf{35}}    & \multicolumn{1}{l|}{\textbf{720}}   \\ \cline{1-5} \cline{7-11} 
vdmj                    & 1940          & 429              & 374            & 2743           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
workspace               & 1438          & 123              & 251            & 1812           &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\textbf{Sum}            & \textbf{6047} & \textbf{1815}    & \textbf{1250}  & \textbf{9112}  &                       &                                              &                                    &                                       &                                     &                                     \\ \cline{1-5}
\end{tabular}
\end{table}

==> 3-Rask/sections/background.tex <==
In this section, we introduce VDMJ which is a tool that provides  language features for \gls{vdm}. 
We further describe the development tool \gls{vscode}, which is used as the \gls{gui} for integration with the language server.
Finally, we describe the standardised protocols \gls{lsp} and \gls{dap} used to decouple the language features from the development tool.

\subsection{VDMJ}
% Page budget: 0.5
% \\Writer: J
% \begin{itemize}
%     \item What is VDMJ.
%     \item How is it useful to support language features. (Lots of reuse).
% \end{itemize}

VDMJ \cite{Battle09} is a command-line tool written in Java, that provides basic language support for the \gls{vdm} dialects VDM-SL, VDM++ and VDM-RT. 
It includes a parser, a type checker, an interpreter, a debugger, a proof obligation generator and a combinatorial test generator with coverage recording, as well as VDMUnit support for automatic testing and user definable annotations.
These are implemented using an extensible \gls{ast} analysed using a visitor framework\cite{Gamma&95}.

Using VDMJ for the language server allows parts of the language support to be reused. 
However, many features of VDMJ are not supported by standardised protocols, thus only a subset of the functionality is used in the language server.

% Since the server is written in Java too it is able to use the language support through integrated function calls whenever the client notifies of changes as opposed to using the command-line interface.
% This allows for a more lightweight and refined solution.

\subsection{Visual Studio Code}
%Page budget: 0.5
%Writer: F
%\begin{itemize}
%    \item What is it? (IDE, Extensible, Platform for GUI).
%    \item How does it relate to LSP and DAP? (Document structure for workspace, comes from the design considerations of VSCode).
%\end{itemize}

\gls{vscode}\footnote{See \url{https://code.visualstudio.com/}} is a free source code editor. 
It has built-in support for the programming languages JavaScript and TypeScript and further enables support for other languages through a rich ecosystem of extensions.
\gls{vscode} uses a folder or workspace system for interacting with a project and a document system for handling the source code files in the project.
This allows \gls{vscode} to be language-agnostic and delegate language specific functionality to an extension. 
Given this design reasoning, a need for the standardisation of decoupling between editor and extension has been identified.
At the time of writing, three different protocols have been developed for this purpose. 
Namely \gls{lsp}\footnote{See \url{https://microsoft.github.io/language-server-protocol/}} (described in \Cref{subsec:lsp}), \gls{dap}\footnote{See \url{https://microsoft.github.io/debug-adapter-protocol/}} (described in \Cref{subsec:dap}) and Language Server Index Format (LSIF)\footnote{See \url{https://microsoft.github.io/language-server-protocol/overviews/lsif/overview/}}.


\subsection{Language Server Protocol}
\label{subsec:lsp}
% Page budget: 1
% \\Writer: J
% \begin{itemize}
%     \item What is it? (and what kind of features does it support.)
%     \item Makes M x N problem into M + N.
%     \item Message format. (Based on generalization of a text document).
% \end{itemize}

Since most \glspl{ide} support a variety of programming languages, \gls{ide} developers face the problem of keeping up with ongoing programming language evolution \cite{Bunder19a}. 
At the same time language providers are interested in providing as many \gls{ide} integrations as possible to serve a broad audience. 
Consequently, integrating every language, $m$, in every \gls{ide}, $n$, leads to a $m \times n$ complexity.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/LSPApproach.pdf}
    \caption[\gls{lsp} approach to language support.]
        {\gls{lsp} approach to language support. Borrowed from \cite{Rodriguez&18}.}
    \label{fig:LSPApproach}
\end{figure}

The \gls{lsp} protocol defines a standardised protocol to be used to decouple a language-agnostic development tool (client) and a language-specific server that provides language features like syntax-checking, hover information and code completion.
This is illustrated in \Cref{fig:LSPApproach}.
The client is responsible for managing editing actions without any knowledge of the language and the server validates the correctness of the source code and reports issues and language-specific information to the client.
To facilitate this the \gls{lsp} protocol communicates using language neutral data types such as document references and document positions.
% \hl{If the communication was to be at language domain level, they would have to make a standardisation of abstract syntax trees and compiler symbols, to be able to use the protocol for multiple languages.
% Thus, communicating using language neutral data types not only allows the protocol to be used for all text based languages, but also simplifies the protocol as it is much simpler to standardise a text document reference or position.}\todo{remove? include it if we use it in future work to explain that support will be trickier using language neutral types}

Many tools support the \gls{lsp} protocol which reduces the time needed to create a client implementation\footnote{See \url{https://microsoft.github.io/language-server-protocol/implementors/tools/}}.
Furthermore, new development tools only have to support the protocol, which can be done with little effort compared to native integration \cite{Bunder19b}. 
Additionally, as the server is separated from the development tool it can be used for multiple tools.
This allows tools to easily support multiple languages and features. 
Thus, by decoupling the language implementation from the editor integration the complexity is reduced to $m + n$.


\subsection{Debug Adapter Protocol}
\label{subsec:dap}
%Page budget: 1
%Writer: F
The \gls{dap} protocol is a standardised protocol for decoupling \glspl{ide}, editors and other development tools from the implementation of a language-specific debugger. 
%It is used to communicate between two processes in a client-server architecture, where the server handles the debug functionality and the client integrates with the development tool.
The \gls{dap} protocol uses language neutral data types, which makes the protocol possible to use for any text-based language.
The debug features supported by the protocol includes: different types of breakpoints, variable values, multi-process and thread support, navigation through data structures and more.

To be compatible with existing debugger components, the protocol relies on an intermediary debug adapter component.
It is used to wrap one or multiple debuggers, to allow communication using the \gls{dap} protocol.
The adapter is then part of a two-way communication with a generic debugger component, which is integrated in a given development environment as illustrated in \Cref{fig:DAPArchitecture}. 
Thus, the protocol reduces a $m \times n$ problem of implementing each language debugger for each development tool into a $m + n$ problem.

\begin{figure}[htb]
    \centering
        \includegraphics[width=0.8\textwidth]{figures/DAP_architecture.pdf}
    \caption[The decoupled architecture where the \gls{dap} protocol is used.]
        {The decoupled architecture where the \gls{dap} protocol is used. }
    \label{fig:DAPArchitecture}
\end{figure}

% The \gls{dap} specification defines a base protocol with three language neutral message types \emph{requests}, \emph{responses} and \emph{events}. 
% The specification further expands on this base to handle communication relating to common debug features.
% As is the case for the \gls{lsp} protocol, the \gls{dap} protocol uses language neutral data types in its communication messages, which makes the protocol possible to use for any text-based language.



==> 3-Rask/sections/conclusion.tex <==
% Page budget: 1-2
% \\Writer: J

% Future work:
% \begin{itemize}
%     \item Improved syntax highlighting
%     \item Additional specification language features
% \end{itemize}

In this paper we have investigated the efforts needed to support \gls{vdm} in \gls{vscode} using the standardised protocols \gls{lsp} and \gls{dap} and our \gls{lsp} extension \gls{slsp}.
Also, we evaluated to which extent the \gls{vdm} language features can be covered by the protocols.

The implementation efforts were estimated using a LoC measure.
In total, the \gls{vscode} extension consists of 1880 LoC, where only 210 are related to the support of the standardised protocols.
This is possible because \gls{vscode} provides generic modules for supporting the protocols.
Similar generic support is found in other \glspl{ide}, we therefore believe that the implementation efforts for these \glspl{ide} are comparable to our results.
The protocol support for VDMJ totals 7855 LoC which we find appropriate as the server allows the language support to be easily reused in other \glspl{ide} as they only have to adhere to the protocols to use the server, which requires little effort compared to creating native support for \gls{vdm}.

In the language feature coverage evaluation we find that only a subset of the \gls{vdm} language features are covered by standard protocols.
To support features related to specification languages, such as \gls{pog} and \gls{ct} we propose the protocol extension \gls{slsp}. 

Going forward we believe that it would be beneficial to also support other specification language features related to validation, verification and translation, using a similar architecture to decouple the language features from the development tool using a language-agnostic protocol.
This would make it easier for multiple development tools to support specification languages, reduce the long term efforts needed to maintain language support, and increase the uptake of specification languages by allowing users to use their preferred development tool.

% From the \gls{lsp} support implemented for VDMJ, consisting of syntax-checking, type-checking and go-to functionality, we believe that most of the editor related features for \gls{vdm} can be supported by the \gls{lsp} protocol.
% However, more work will have to be carried out on the server to support the full \gls{lsp} protocol.
% Furthermore, we find that the \gls{dap} protocol is able to support debugging of VDM specifications.

% Going forward we believe that it would be beneficial to also support other specification language features related to validation, verification and translation, using a similar architecture to decouple the language features from the development tool using a language-agnostic protocol.
% This would make it easier for multiple development tools to support specification languages, reduce the long term efforts needed to maintain language support, and increase the uptake of specification languages by allowing users to use their preferred development tool.

% \todo[inline]{Maybe move the below part to its own section adding more details about POG and CT work?}
% We are currently investigating if we can support the specification language specific features using a language-agnostic protocol.
% To achieve this, we are proposing and currently developing an extension to the standard \gls{lsp} protocol.

% We expect it to be possible to support the additional specification language features.
% The current work carried out in this direction supports both \gls{pog} and \gls{ct}.
% Concurrently with the protocol development a \gls{poc} is also being developed to investigate the feasibility of utilising the protocol to support \gls{vdm} features in another \gls{ide} than Overture.
% The \gls{poc} is made as an extension to \gls{vscode} which adds support not only for editor features but also for \gls{pog} and \gls{ct}.

% By the time of the presentation of the paper we expect to be able to show support in \gls{vscode} for editorial features, \gls{pog} and \gls{ct}, and possibly translation and a suggestion for how to support theorem proving.

==> 3-Rask/sections/introduction.tex <==
%Page budget: 1
%Writer: Hugo 

The \gls{vdm} is one of the approaches to follow, when applying formal methods during the development of computer systems.
%
The method prescribes the development of digital/computer models of the system under development in one of the the \gls{vdm} specification languages and dialects. If the models are described in an executable subset it is then possible to execute and analyse them to reach a high-fidelity system description, which is then subsequently used to produce code in the  programming languages used to operate the system implementation.

To support all the steps involved in the development of a \gls{vdm} model, there are several tools and \glspl{ide} supporting the variety of \gls{vdm} specification languages and dialects to different levels \cite{Larsen&16}.
%
VDMTools were the first available commercial tool developed in the  mid-1990s \cite{3-Rask:Larsen01}. Then Overture \cite{3-Rask:Larsen&10a} brought free and open-source support to \gls{vdm} in 2005, and many others are now available \cite{Oda&15,Tran&19}.

The Overture tool is one of the most complete and popular \glspl{ide} for \gls{vdm}. It consists of multiple plugins that extend the Eclipse \gls{ide}, which appeared in the 2000s.
Eclipse is the most popular\footnote{See \url{https://pypl.github.io/IDE.html}} in its class, but it is being challenged by a new contender, the \gls{vscode}\footnote{See \url{https://code.visualstudio.com/}} editor, which is based on Electron\footnote{See \url{https://www.electronjs.org/}.} and fully leverages web technologies.
%
%Visual Studio Code popularity is growing exponentially, 
%and is now the third most searched free and open-source editor, and many expect it to be widely adopted by the new generations of developers\todo{cite?}. 
%
Although not an \gls{ide}, \gls{vscode} modernized the \gls{ide} world, with  the introduction of the \gls{lsp}\footnote{See \url{https://microsoft.github.io/language-server-protocol/}.} and the \gls{dap}\footnote{See \url{https://microsoft.github.io/debug-adapter-protocol/}.}, which enable the development of \gls{ide} features in a general manner. With the two protocols the editor becomes indistinguishable of an \gls{ide}, and the implementation code becomes reusable and better maintainable.
However, the Overture language core does not implement the LSP and DAP protocols, so the effort required to move towards \gls{vscode} is significant, but we expect it to pay off in the long run.

In this paper we investigate the efforts needed to support \gls{vdm} in \gls{vscode} with as much as possible of the support using the standardised protocols \gls{lsp} and \gls{dap}.
To support specification lanuage features not found in programming languages we propose an extension to \gls{lsp}, \gls{slsp}.
As part of the investigation we have extended VDMJ such that it can be used as a language server that supports both these protocols. 
The server supports syntax-checking, type-checking and go-to functionality using the \gls{lsp} protocol, debugging by using the \gls{dap} protocol, and \gls{pog} and \gls{ct} using the \gls{slsp} protocol.
We have also developed a \gls{vscode} extension which connects to the language server in order to provide the language features in the \gls{ide}.
In addition, we have investigated which features are required to provide full language support for specification languages and which of these are supported by the protocols.
% We are currently working to determine the feasibility of fully decoupled language support from the \gls{ide} for formal specification languages (like the VDM dialects), this ongoing work is shortly described in the paper.
% \todo{Maybe we can substitute this last sentence by pointing the paper also documents the studies made to plan for the future developments (ongoing work), thus wrapping the paragraph.}The extension provides the client side for the protocols and syntax highlighting trough the use of Textmate grammars.

Our work departs from a previous proof of concept, and adds further support for the LSP protocol, support for all the VDM dialects, support for the DAP protocol and support for the \gls{slsp} protocol. 
In addition, this is the first research paper on the topic, and we foresee more publications to emerge from the works towards fully supporting VDM development using \gls{vscode}.
We believe the resulting extensions will become the next in line supporting \gls{vdm} development. A modern and robust IDE, which development starts now. 

The remaining parts of this paper starts with an overview of the background necessary to understand this paper in \Cref{3-Rask:sec:background}. Afterwards \Cref{sec:Implementation} explains how the standard protocols \gls{lsp} and \gls{dap} have been used to implement the core of the \gls{vscode} support for \gls{vdm}. This is followed by \Cref{sec:Evaluation} which is evaluating the efforts that has been conducted. 
In \Cref{sec:relatedWork} we describe related work.
Finally, \Cref{3-Rask:sec:conclusion} provides concluding remarks and future work.


==> 4-Bogomolov/Sections/RobottiDSE-old.tex <==
\section{Robotti Pilot Study: Design Space Exploration}
\label{sec:RobottiDSE}

\subsection{Robotti Pilot Study: Experiment Overview}

The objective of the Robotti pilot study was to calibrate Robotti model parameters against results obtained from a physical robot trial which contained robot position ($x$, $y$ coordinates) at time $t$ while performing a specific maneuver.

\begin{itemize}
	\item[--] explain each block!
\end{itemize}

\begin{figure}
	\centering
	\begin{tikzpicture}[every node/.append style={draw=black!60, inner sep=5pt, minimum size=50pt, fill=gray!5}, scale=\textwidth]
	
	\node[draw=black, fill=gray!5, minimum size = 40pt] (centre) at (0,0) {MM};
	
	\node[draw=none, fill=none, minimum size = 10pt, right = 1 cm of centre] (param) {$\mathsf{[cAlpha, mass, mu]}$};
	
	\node[draw=black, fill=gray!5, minimum size = 40pt, above = 1.5 cm of centre] (centre2) {SN};
	\node[draw=none, fill=none, minimum size = 40pt, left = 1 cm of centre2] (fakecentre2) {};
	
	\node[draw=black, circle,  fill=gray!5, minimum size = 10pt, below = 1.5 cm of centre] (sum)  {+};
	\node[draw=none, fill=none, minimum size = 40pt, left = 1.25 cm of sum] (mm) {};
	
	\draw[->] (centre) -- (sum) node[draw=none, fill=none,midway, minimum size = 5pt, right] (ref) {\footnotesize{$\mathsf{results[s_n].csv}$}};
	\draw[<-] (centre) -- (centre2) node[draw=none, fill=none,midway, minimum size = 5pt, right] (ref) {\footnotesize{$\mathsf{steering\_inputs[s_n].csv}$}};
	\draw[] (centre2.west) -- (fakecentre2.east) -- (mm.east) node[draw=none, fill=none,midway, minimum size = 5pt, left] (ref) {\footnotesize{$\mathsf{gps\_pos[s_n].csv}$}};;
	\draw[->] (mm.east) -- (sum.west);
	\draw[->] (param) -- (centre);
	
	
	\node[draw=none, fill=none, minimum size = 40pt, left = 4 cm of centre2, yshift=-7cm] (corner1) {};
	\node[draw=none, fill=none, minimum size = 40pt, left = 4 cm of centre2, yshift=0.5cm] (corner11) {};
	\node[draw=none, fill=none, minimum size = 40pt, right = 4 cm of centre2, yshift=-7cm] (corner2) {};
	\node[draw=none, fill=none, minimum size = 40pt, right = 4 cm of centre2, yshift=0.5cm] (corner21) {};
	
	\draw[dashed] (corner21.north) -- (corner11.north)-- (corner1.north) -- (corner2.north) -- (corner21.north);
	
	
	
	\node[draw=none, fill=none, rotate=0, right = .1 cm of sum] {$\mathsf{Algorithm \; 1}$};
	
	\node[draw=black, fill=gray!5, minimum size = 40pt, below = 1 cm of sum] (op) {OP};
	\node[draw=none, fill=none, minimum size = 0pt, above = .55 cm of op] (op2) {};
	\draw[->] (op2) -- (op) node[draw=none, fill=none,midway, minimum size = 5pt, right] (ref) {\footnotesize{$\mathsf{dse\_results.csv}$}};
	
	\node[draw=none, fill=none, rotate=0, right = .1 cm of op] {$\mathsf{Algorithm \; 2}$};
	
	\node[draw=none, fill=none, minimum size = 10pt, left = .8 cm of op] (param2) {$\mathsf{[cAlpha, mass, mu]}$};
	
	\draw[->] (op) -- (param2);
	
	\node[draw=none, fill=none, rotate=0, left = .7 cm of centre2, yshift=5mm] {$\mathsf{DSE\_Configuration.json}$};
	
	%\node[draw=none, fill=none, minimum size = 0pt, above = .5cm of centre] (centre2) {};
	
	%	\node[draw=black, fill=gray!5, minimum size = 40pt, below = 2cm of centre] (pareto) {PAR};
	
	%	\node[draw=black, fill=gray!5, minimum size = 40pt, left = 5cm of pareto] (optimization) {OPT};
	%	\node[draw=none, fill=none, minimum size = 40pt, left = .5 cm of optimization] (optimization2) {$\mathsf{params}$};
	
	%	\node[draw=none, fill=none, minimum size = 0pt, left = 1.5cm of pareto] (pareto2) {};
	
	
	
	
	
	%	\node[draw=black, circle,  fill=gray!5, minimum size = 10pt, right = 2 cm of centre] (sum)  {+};
	
	
	
	
	%	\node[draw=black, fill=gray!5, minimum size = 10pt, text width=35mm, left = 3cm of centre] (scenario) {scenarios = [s1, s2, ...]};
	
	%\node[draw=black, fill=gray!5, minimum size = 10pt, text width=35mm,below = .3 cm of scenario] (parameters) {parameters = [p1, s2, ...]};
	
	%	\draw[->] (scenario) -- (centre) node[draw=none, fill=none,midway, minimum size = 5pt, above] (ref) {\footnotesize{$\mathsf{steering\_input[s_n].csv}$}};
	
	
	%	\draw[] (scenario.north) |- (centre2.west) node[draw=none, fill=none,midway, minimum size = 5pt, above, xshift=5cm] (ref) {\footnotesize{$\mathsf{gps\_pos[s_n].csv}$}};
	%	\draw[->] (centre2.west) -| (sum.north) node[draw=none, fill=none,midway, minimum size = 5pt, above] (ref) {};
	
	%	\draw[->] (sum.south) |- (pareto.east) node[draw=none, fill=none,midway, minimum size = 5pt, above, xshift=-12mm] (ref) {\footnotesize{$\mathsf{mean\_track\_error}$}};
	
	
	\end{tikzpicture}
	\caption{The DSE analysis workflow overview of the Robotti pilot study}
	\label{fig:method}
\end{figure}

\subsection{Robotti Pilot Study: DSE Configuration and Objective Function}
\def\Plus{\texttt{+}}

Performing design space exploration requires defining an objective function (and script) and DSE configuration which will guide exploration process, quantify and rank a series of co-simulations with varied parameter values. The DSE configuration file for the Robotti pilot study

\begin{lstlisting}[language=json,firstnumber=1, caption = {Robotti pilot study DSE configuration file}]
{
"algorithm": {"type":"exhaustive"},

"objectiveDefinitions":
	{"externalScripts":{"robottiCrossTrack": {"scriptFile":"robottiCrossTrack.py",
"scriptParameters":{
					  "1":"time",
					  "2":"{Robotti}.RobottiInstance.y3_out",
					  "3":"{Robotti}.RobottiInstance.y4_out"}
					  },
"parameters":{
"{Robotti}.RobottiInstance.cAlphaF":[20k,24.5k,29k,33.5k,38k],
"{Robotti}.RobottiInstance.mu":[0.3,0.4,0.5,0.6,0.7],
"{Robotti}.RobottiInstance.m_robot":[1k,1.5k,2k,2.5k,3k]
			 },
}

\end{lstlisting}

\textbf{configuration file}

The tunning of Robotti model parameters was decided to be based on mean deviation between recorded and simulated robot positions for a specific maneuver. The deviation measure has been implemented with a root-mean-squared-error metric which measures mean a distance between two series of coordinates and can be expressed as Equation 1.

\begin{equation}
\mathsf{RMSE} = \dfrac{\sum\limits_{i=1}^{n} \sqrt{(x_{i2} - x_{i1})^{2} + (y_{i2} - y_{i1})^{2}}}{n}
\end{equation}

The measure was implemented as a Python script (described in Algorithm 1) which imports $\mathsf{gps\_pos.csv}$ and simulation result $\mathsf{results.csv}$ files. The $\mathsf{cross\_track\_error}$ function then firstly applies a numerator part of the root-mean-squared-error measure for corresponding rows of imported files and once every position entry of the  $\mathsf{gps\_pos.csv}$ has been compared function computes and returns a mean error value. The measured objective value with the name of objective name are then stored in the $\mathsf{objective.json}$ file with an internal tool function $\mathsf{writeObjectiveToOutfile}$.  \vspace{2mm}

\begin{algorithm}[h]
\caption{Root mean squared error objective function algorithm script}
\begin{algorithmic}[1]
\item $\mathsf{[Skeleton \: Code]}$
\item
\item $\mathsf{import \; gps\_pos.csv \; as \; gps}$
\item $\mathsf{import \; results.csv \; as \; results}$
\item
\item \textbf{def} $\mathsf{cross\_track\_error(gps, results):}$
\item \quad $\mathsf{result = [\: ]}$
\item \quad \textbf{for} $\mathsf{p}$ \textbf{in} \textbf{range}$[0, \; \mathbf{len}(\mathsf{gps})]$
\item \quad \quad $\mathsf{result}$.$\mathbf{append[}$$\mathsf{sqrt((gps[x_p] - results[x_p])^{2}  + (gps[y_p] - results[y_p])^{2}) }$]	
\item \quad $\mathsf{mean\_error}$ =  $\mathbf{sum}(\mathsf{result}) / \mathbf{len}(\mathsf{gps})$
\item \quad \textbf{return} $\mathsf{mean\_error}$
\item
\item  $\mathsf{objective\_result}$ = $\mathbf{cross\_track\_error}$$\mathsf{(gps, results)}$
\item \textbf{writeObjectiveToOutfile}$(\mathsf{objectives.json}, \mathsf{objectiveName}, \mathsf{objective\_result})$
\end{algorithmic}
\end{algorithm}

\newpage
\subsection{Robotti Pilot Study: Optimum Parameter Search}

The main objective of this exercise is finding the best fitting parameters of the model given the different simulated and measured scenarios. The problem of finding the best fitting parameters can be considered as optimization (function minimization) problem where a function in Robotti pilot study to be minimized maps parameter values to mean track value error computed by Algorithm 1.

The function we intend to minimize is given in Equation 1 where $\mathcal{E}_{s}$ is a set of mean track error functions constructed from the simulated scenarios and parametrised by a scenario ${s \in \{sin1, sin2, sin3 \cdots \}}$ and constrained domain $dom(\mathcal{E})$.

\begin{equation}
\begin{aligned}
f^{-} = & arg \; \min \sum_{s \in S} \mathcal{E}_{s}(\alpha, m, \mu) \; where \: dom(\mathcal{E}) :\\
& \alpha \in \{20000, 24500, 29000, 33500, 38000\} \\
& m \in \{1000,1500,2000,2500, 3000\}  \\
& \mu \in \{0.3,0.4,0.5,0.6,0.7\}
\end{aligned}
\end{equation}

The minimization function has been implemented as a Python script and is described in Algorithm 2 listing where the main function $\mathsf{searchParameters()}$ explores all permutations of parameter values. \vspace{2mm }

\begin{algorithm}[h]
	\caption{Total mean track error value minimization algorithm}
	\begin{algorithmic}[1]
		\item $\mathbf{def}$ $\mathsf{getResults}(cAlpha, mass, mu):$
		\item \quad \quad $\mathsf{total\_error\_value \: = 0.0}$
		\item \quad \quad \quad $\mathbf{for}$ $\mathsf{s}$ $\mathbf{in}$ $\mathsf{[s_0, s_1, \cdots s_n]}$
		\item \quad \quad \quad \quad$\mathsf{total\_error\_value \: \Plus=  \mathcal{E}_s(cAlpha, mass, mu)}$
		\item \quad \quad $\mathbf{return}$ $\mathsf{total\_error\_value}$
		\item
		\item $\mathbf{def}$ $\mathsf{searchParameters}():$
		\item \quad \quad $\mathsf{minimum}$ = $\mathsf{init}$
		\item \quad \quad$\mathsf{cAlphaF}$ = $[20000, 24500, 29000, 33500, 38000]$
		\item \quad \quad$\mathsf{mass}$ = $[1000,1500,2000,2500, 3000]$
		\item \quad \quad $\mathsf{mu}$ = $[0.3, 0.4, 0.5, 0.6, 0.7]$
		\item
		\item \quad \quad $\mathbf{for}$ $i_0$ $\mathbf{in}$ $\mathbf{range}[\mathsf{0, len(cAlphaF)}]$
		\item \quad \quad \quad \quad $\mathbf{for}$ $i_1$ $\mathbf{in}$ $\mathbf{range}[\mathsf{0, len(mass)}]$
		\item \quad \quad \quad \quad \quad \quad $\mathbf{for}$ $i_2$ $\mathbf{in}$ $\mathbf{range}[\mathsf{0, len(mu)}]$
		\item \quad \quad \quad \quad \quad \quad \quad \quad$\mathbf{if} (\mathsf{getResults(cAlphaF[i_0], mass[i_1], mu[i_2])} < \mathsf{minimum}): $
		\item  \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad $\mathsf{minimum}$ = $\mathsf{getResults(cAlphaF[i_0], mass[i_1], mu[i_2])}$
		\item  \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad $\mathsf{parameters}$ = $\mathsf{cAlphaF[i_0], mass[i_1], mu[i_2]}$
		\item
		\item \quad \quad $\mathbf{return}$ $\mathsf{(minimum, parameters)}$
	\end{algorithmic}
\end{algorithm}

%\begin{figure}
%	\includegraphics[width=.8\paperwidth]{scenario1.png}
%	\caption{text}
%	\label{sec6: scenario1}
%\end{figure}

The results of this exercise are summarised in the Table 1.
\begin{center}
	\begin{table}[h!]
		\begin{tabular}{ c | c | c | c | c}
			\hspace{5mm} $\mathsf{scenario}$ \hspace{5mm} & \hspace{5mm} $\mathsf{min}$ \hspace{5mm} & \hspace{5mm} $\mathsf{max}$ \hspace{5mm} & \hspace{5mm} $\mathsf{mean}$ \hspace{5mm} & \hspace{5mm} $\mathsf{computed}$ \hspace{5mm} \\
			\hline
			\hspace{5mm} $\mathsf{sin1.csv}$ \hspace{5mm} & 1.188 & 1.371 & 1.323 & 1.318 (\textcolor{green}{-5E-3}) \\
			\hspace{5mm} $\mathsf{sin2.csv}$ \hspace{5mm} & 1.680 & 1.960 & 1.884 & 1.891 (\textcolor{red}{+7e-3}) \\
			\hspace{5mm}  $\mathsf{sin3.csv}$ \hspace{5mm} & 2.139 & 9.218& 4.561 & 5.486 (\textcolor{red}{+9.25e-1}) \\
			\hspace{5mm} $\mathsf{speed\_step1.csv}$ \hspace{5mm} & 0.742 & 0.742 & 0.742 & 0.742 (\textcolor{red}{})  \\
			\hspace{5mm} $\mathsf{speed\_step2.csv}$ \hspace{5mm} & 0.578 & 0.578 & 0.578 & 0.578 (\textcolor{red}{})\\
			\hspace{5mm} $\mathsf{speed\_step3.csv}$ \hspace{5mm} & 0.482 & 0.482 & 0.482 & 0.482  (\textcolor{red}{})\\
			\hspace{5mm} $\mathsf{turn\_ramp.csv}$ \hspace{5mm} & 2.056 & 2.222 & 2.188 & 2.194 (\textcolor{red}{+6e3})\\
			\hspace{5mm} $\mathsf{turn\_ramp2.csv}$ \hspace{5mm} & 1.408 & 1.560 & 1.525 & 1.542 (\textcolor{red}{+1.7e2}) \\
			\hspace{5mm} $\mathsf{turn\_ramp3.csv}$ \hspace{5mm} & 2.233 & 2.497 & 2.431 & 2.456  (\textcolor{red}{+2.5e2})\\
			\hspace{5mm} $\mathsf{speed\_ramp1.csv}$ \hspace{5mm} & 0.307 & 5.120 & 3.244 & 0.312 (\textcolor{green}{-2.932}) \\
			\hspace{5mm} $\mathsf{speed\_ramp2.csv}$ \hspace{5mm} & 0.367 & 3.965 & 3.328 & 0.430 (\textcolor{green}{-2.898})\\
			\hspace{5mm} $\mathsf{speed\_ramp3.csv}$ \hspace{5mm} & 0.431 & 1.460 & 1.214 & 0.431 (\textcolor{green}{-1.1709})
		\end{tabular}
		\vspace*{5mm}
		\caption{The summary of optimization results and best fitting parameters: $\mathsf{mean\_cross\_track\_error_{total}}$ = 17.865 with $\mathsf{CAlphaF}$ = 38000, $\mathsf{mass}$ = 1000,  $\mathsf{\mu}$ = 0.3}
	\end{table}
\end{center}

\begin{figure}
\includegraphics[width=.7\paperwidth]{Figures/correlation.png}
\end{figure}


\begin{figure}[t]
	\centering
	\begin{subfigure}{0.45\columnwidth}
		\includegraphics[width=\columnwidth]{Figures/Sin1.png}
		\caption{}\label{Figure15a}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.45\columnwidth}
		\includegraphics[width=\columnwidth]{Figures/Turn_Ramp1.png}
		\caption{}\label{Figure15b}
	\end{subfigure}%
	\caption{blah blah \textbf{(a)} something something \textbf{(b)}.}
	% \vspace{-2\baselineskip}
	\label{Figure15}
\end{figure}

==> 4-Bogomolov/Sections/RobottiResults.tex <==
\section{Robotti Pilot Study: Results}
\label{sec:results} 

\begin{itemize}
\item Present DSE outcomes in an appropriate way? 
\end{itemize}

==> 4-Bogomolov/intocpstoolchain.tex <==
%\fbox{Casper}

\begin{figure}
	\begin{center}
    \includegraphics[width=0.75\linewidth]{Figures/Toolchain}
	\caption{Schematic of the INTO-CPS tool chain.	\label{fig:toolchain}}
    \end{center}
\end{figure}

The INTO-CPS Tool Chain~(Figure~\ref{fig:toolchain})
supports an MBSE approach to CPS development that allows the Discrete-Event (DE) formalisms used to express cyber processes and Continuous-Time (CT) formalisms used for physical processes to co-exist in a common simulation framework. The act of collaboratively simulating these constituent models such that a simulation of a CPS is achieved is referred to as coupled simulation (co-simulation)~\cite{Gomes&18}. A co-simulation is generally carried out by simulating the individual models while exchanging data and managing the progress of time between them.

Co-simulation requires the orchestration of a range of discipline-specific simulation tools~\cite{Bastian&11,INTOCPSD3.3a}.
%In order to conduct a co-simulation, and thereby combine the different disciplines, it can be necessary to utilise several specialised tools for simulating a given model~\cite{Bastian&11,INTOCPSD3.3a}.
The Functional Mock-up Interface (FMI) \cite{FMIStandard2.0.1} is an approach to generalising the simulation interface of models that are to participate in a co-simulation. FMI provides and describes a C-interface and the structure of a model description file. A model implementing
this C-interface and providing a model description file is referred to as a
Functional Mock-up Unit (FMU) and it can contain its own solver. The INTO-CPS
Toolchain is based on FMI 2.0 for its simulation capabilities.

The main user interface to the INTO-CPS tool chain is the INTO-CPS Application \cite{Macedo&20} which has been developed on the Electron platform.
%The rest of this section describes individual tools and concepts directly
%related to the INTO-CPS Toolchain.

The INTO-CPS Co-simulation Orchestration Engine (COE), called Maestro~\cite{Thule&19}, manages the FMUs in accordance with
various co-simulation algorithms. It is configured by a \emph{multi-model} and a \emph{configuration}. The multi-model defines the FMUs participating in
a co-simulation, the dependencies between them, and their parameters. The
configuration specifies the co-simulation execution including details such as logging and step size (i.e., the time interval between value
exchanges between the FMUs).
%The actual realisation of Maestro is a jar file called \texttt{coe.jar}.

The tool chain also supports Design Space Exploration (DSE). This is the process of systematically executing co-simulations with a variety of values for specified design parameters, with the goal of maximising an objective such as energy efficiency or a performance measure~\cite{Broenink&12b,INTOCPSD3.3a} and part of the INTO-CPS Toolchain.

The tool chain is neutral about the sources of FMUs, but it has been instantiated with several formalisms and simulation engines. For example, DE models can be developed in the Overture tool~\cite{Larsen&10a} which supports a dialect of the Vienna Development Method's modelling language for Real Time systems (VDM-RT~\cite{Verhoef&06b}). Using Overture and the extension
overture-fmu\footnote{\url{https://github.com/overturetool/overture-fmu}} one can
export FMUs from a VDM-RT project~\cite{Thule&18,Hasanagic&19}. CT models have been developed using 20-sim\footnote{\url{https://www.20sim.com}}, which also can export conformant FMUs.

%The final piece of the puzzle is the development of the constituent models
%expressed as FMUs. The development of DE models is carried out using the
%eclipse-based open-source tool called Overture \cite{Larsen&10a}. It includes a dialect of the Vienna
%Development Method (VDM) called VDM Real Time (VDM-RT) with various real time
%concepts, i.e.\ clocks \cite{Verhoef&06b}. Using Overture and the extension
%overture-fmu\footnote{\url{https://github.com/overturetool/overture-fmu}} one can
%export FMUs from a VDM-RT project~\cite{Thule&18,Hasanagic&19}. The development of CT models is
%carried out using the tool 20-sim\footnote{\url{https://www.20sim.com}}. This tool can be used for modelling and
%analysing dynamic systems and is capable of exporting FMUs that represent a
%given model.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 5-Tola/figures/case_study.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=0.7\textwidth]{images/case_study.pdf}
    \caption{An illustration of the autonomous combine harvester that is used as the case study in this paper.}
    \label{fig:case_study}
\end{figure}

==> 5-Tola/figures/cosim_fmu.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{images/cosim_fmu.pdf}
    \caption{An illustration of how co-simulation can combine FMUs developed using different tools, and also some of the main files inside an FMU.}
    \label{fig:cosim_fmu}
\end{figure}

==> 5-Tola/figures/evidence_scenarios.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{images/evidence_scenarios.pdf}
    \caption{An illustration of how the scenarios related to specific evidence are created, and how these scenarios define the co-simulation parameters of the models used. The models are created using domain knowledge about the system, or by reusing other models. The co-simulation results of the model with specific parameters, can then be used to prove that the system is safe, and therefore used as evidence in the safety case. The scenarios are defined using domain knowledge or researched articles. The scenarios are usually defined with values of worst case scenarios.}
    \label{fig:evidence_scenarios}
\end{figure}

==> 5-Tola/figures/gsn_elems.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.85\textwidth]{images/gsn_elems.pdf}
    \caption{The relevant elements used in \textit{GSN}. The figure is inspired from~\cite{Kelly&04}.}
    \label{fig:gsn_elems}
\end{figure}

==> 5-Tola/figures/gsn_to_model.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/gsn_to_model.pdf}
    \caption{The steps performed when creating models. The knowledge from the safety goals in the GSN and the hazardous events is used to define test scenarios. In order to co-simulate these test scenarios, models of different parts of the system must be created by reading articles, using domain knowledge or using existing models.}
    \label{fig:gsn_to_model}
\end{figure}

==> 5-Tola/figures/main_stage_sc.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/main_stage_sc.pdf}
    \caption{The relevant main stages of a safety case.}
    \label{fig:main_stage_sc}
\end{figure}

==> 5-Tola/figures/process_evidence.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{images/process_evidence.pdf}
    \caption{An illustration of the possible techniques for producing evidence that can be used in a safety case. The specific technique must be determined after defining the safety goals.
    Note that evidence technique A also requires model validation in order to be able to use the co-simulation results as evidence.}
    \label{fig:process_evidence}
\end{figure}

==> 5-Tola/figures/seq_gsn_to_evidence.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{images/seq_gsn_to_evidence.pdf}
    \caption{The steps performed when producing evidence using co-simulation. These steps are performed after create a safety case analysis, where a GSN is created and the evidence that can be co-simulated is already determined. The input of this stage, is the GSN with the evidence that must created, and the output is either evidence that can be used in the GSN, or knowledge of improvements to the system that must be made.}
    \label{fig:seq_gsn_to_evidence}
\end{figure}

==> 5-Tola/sections/background.tex <==
\section{Background} \label{sec:background}

This section describes the required background knowledge to understand the subsequent sections in this paper.

\subsection{Case Study} \label{sec:background:case_study}

The case study is based on a system where the goal is to develop a combine harvester, which can autonomously drive within the boundaries of a crop field and harvest crops, without the need for a driver controlling the vehicle.

Figure~\ref{fig:case_study} illustrates how the environment of the autonomous combine harvester may look, including a number of the sensors that will be used in the system. The figure also demonstrates how animals may hide in between the crops, which in some cases can be difficult to detect. The system can potentially injure or kill living creatures in the field, damage the harvested crops (if the vehicle runs over an animal, the harvested crops will be contaminated), or catch fire~\cite{Val&19}. These are few of the reasons that this system is categorised as safety-critical. The motivation for using this system as the case study when researching how to incorporate co-simulation in the development of a safety-critical system, is:

\begin{itemize}
    \item It is challenging to test the system in the different atmospheric environments where the conditions cannot be controlled, such as extremely windy, rainy, or foggy. 
    \item It is unethical to test the system with living creatures on the field, to determine if the system operates as it should under these specific circumstances.
\end{itemize}

\input{figures/case_study}

% If the sensors are not used any more throughout the paper, then remove them from the figure and the text

% ----------------------------------------------------------------------------------------------------
\subsection{Safety Case}

The safety of a safety-critical system must typically be demonstrated to a government regulatory body, by creating a safety case~\cite{Sommerville96}, which is defined as~\cite{Bishop&98}:
\begin{quote}
    \say{\textit{A documented body of evidence that provides a convincing and valid argument that a system is adequately safe for a given application in a given environment.}}
\end{quote}

\noindent The three main elements used in a safety case are~\cite{Bishop&98,Kelly&04}:
\begin{description}
    \item[Claim:] a safety requirement or claim about the system, for example \say{System X is safe}.
    \item[Evidence:] used to support the claims about the safety of the system, for example physical tests of the system operating safely in specific environmental conditions.
    \item[Argument:] used to describe how the evidence supports the safety claims.    
\end{description}

The main stages of a safety case, that are relevant for this paper, are illustrated in Figure~\ref{fig:main_stage_sc}. The information obtained at each stage is used in the following stages. For example, the system description can be used in the process of deriving hazards. A hazard is defined as a system state, where the system may potentially damage its surroundings. It is important to note that a system can be in a hazardous state without causing an accident~\cite{Sommerville96}. 

The hazard analysis stage consists of identifying hazards and their root causes. Different methods exist for finding root causes of hazards, and usually multiple methods will be used. In this paper we chose to only use one method, \textit{fault-tree analysis}, due to its simplcity and graphical view. It is a top-down approach, starting with a hazard and moving down towards potential events that may lead to the occurrence of the hazard. In the fault-tree analysis approach, events that may lead to a hazard are presented graphically using logical gates, such as AND and OR gates~\cite{Sommerville96}.

The risk of each of the identified hazards is then assessed by determining the severity and likelihood of the hazards~\cite{Despotou&12}. The determined risk of each hazard is then used to order the hazards from highest to lowest risk, and thereby determine the acceptable cost of reducing the risk of a hazard~\cite{Sommerville96}\textcolor{red}. 

\input{figures/main_stage_sc}

One of the existing safety case processes, is to develop the system first and then create the safety case. The disadvantage of this process is that if safety issues are found after the development of the system, then a system redesign may be necessary. Therefore, another process has been adopted, which is the phased safety case process, where the system and safety case are both developed simultaneously. This process is beneficial to use when a novel safety argument is being used, which is the case in this paper. There are typically three main phases to be developed in the phased safety case, Preliminary, Interim and Operational. The details of the safety case increase with each phase~\cite{Kelly2003}. We only consider the Preliminary safety case in this paper.

% ----------------------------------------------------------------------------------------------------

\subsection{Goal Structuring Notation}

Creating explicit and clear safety arguments using plain text is not always a simple task, and can therefore end in misinterpretations by the regulator. The Goal Structuring Notation (GSN) attempts to solve these potential problems by using a graphical structure, that shows the connections of arguments, safety claims and evidence. 

The relevant GSN elements used in this paper are illustrated in Figure~\ref{fig:gsn_elems}, where the \textit{goal}, \textit{solution} and \textit{strategy} are equivalent to the \textit{safety objective}, \textit{evidence} and \textit{argument} in a safety case, respectively~\cite{Kelly&04}. The \textit{away goal} uses a claim from another module to support the argument in the current module~\cite{GSNCommunityStandard}. The usage of an \textit{away goal} in a GSN for arguing that a simulation tool adequately models the environmental conditions affecting part of a system, can be found in~\cite{Sun&09a}. This method of argumentation, using an \textit{away goal}, is also used in this paper.


\input{figures/gsn_elems.tex}


%----------------------------------------------------------------------------------------------------

\subsection{Modelling and Co-simulation}

A model is defined by J. Van Amerongen as~\cite{Amerongen10}:

\begin{quote}
\say{\textit{A simplified description of a system, just complex enough to describe or study the phenomena that are relevant for our problem context.}}
\end{quote}

\noindent As Amerongan explains, a model should be a simple representation of a system, that is easy enough to understand, but also complex enough to include the important characteristics of the system~\cite{Amerongen10}.

Performing simulations of the model with various parameters allows testing the model under different conditions. A challenge of obtaining a simulation of a complete system is that they are composed of several parts; often modelled using different mathematical formalisms. For example, the combine harvester consists of software, electrical and mechanical parts. Co-simulation allows to use models developed in different tools and execute them simultaneously~\cite{5-Tola:Gomes&18}, where a co-simulation engine is responsible for exchanging the data between the different models~\cite{Fitzgerald&13a}. 

For the co-simulation engine to be able to communicate with the models, each model must implement an interface, such as the Functional Mock-up Interface (FMI). A model that implements the FMI is called a Functional Mock-up Unit (FMU)~\cite{FMIStandard2.0}. Figure~\ref{fig:cosim_fmu} gives an idea of how FMUs developed using different tools can be run in a co-simulation, and also illustrates the main files within in an FMU.
An FMU encapsulates a model as a black box with only the necessary parameters, inputs, outputs and binaries exposed in the interface. This allows Original Equipment Manufacturers (OEMs) to share models of their equipment, and at the same time protect their intellectual property~\cite{FMIStandard2.0}. 


\input{figures/cosim_fmu.tex}


==> 5-Tola/sections/conclusion.tex <==
\section{Concluding Remarks and Future Work} \label{sec:conclusion}


This paper has demonstrated guidelines for incorporating co-simulation into the process of developing a safety case using FMI-based co-simulation. This was demonstrated by applying the process to a case study of an autonomous combine harvester. 


Co-simulation is a strong tool for experimenting with system behaviour, when the system consists of software, electrical and mechanical parts that work together. It is especially relevant to use in the safety case of a complex system, where physical tests of the system are either unethical or challenging to perform. The combine harvester was beneficially co-simulated in scenarios such as dense fog and heavy rain, which are conditions that cannot be controlled in the physical world. The co-simulation was visualized, allowing to create videos of the results, which can advantageously be presented to the regulatory bodies, to help them easier understand how the safety mechanisms ensure system safety under specific conditions.



Different techniques for producing evidence exist, as illustrated in Figure~\ref{fig:process_evidence}, where it is important to consider which technique is most suitable to use depending on the nature of the problem. Looking at co-simulation, the time spent on modeling, co-simulating, analyzing the results and validating the models used, is important to consider. In some cases co-simulation may require too much time, and there may be other techniques that can formally prove the safety of the system, such as a mathematical proof. 


This paper has shown how co-simulation can be used to demonstrate that the design of a system has adressed the identified hazards. This was achieved by running co-simulations of a system model in different hazardous conditions, and using the co-simulation results as evidence in the GSN of a safety case. 


\input{figures/process_evidence}


\subsection*{Future Work}
The work presented in this is based on a specific case study with focus on one hazard, and therefore there are multiple potential areas that can be researched:

\begin{description}
    \item[Extend process:] The process could be extended to both interim and operational safety cases, potentially providing guidelines on how the model fidelity can be increased between each phase. % software from true system can potentially be used in the operational safety case
    \item[Amount of parameters per scenario:] Determining how many parameters should be experimented with is important, to ensure sufficient results for evidence, but also avoid running an endless amount of tests. % we mainly focused on using worst case values
    \item[Model validation:] The model used in this project must be validated, and the methods used to validate it can be explained. Choosing the specific scenarios and parameters to use during validation should be part of this research.
    \item[Evaluate process on other systems:] Using this process on other types of systems, such as medical devices which require human operators, could demonstrate if the process can directly be transferred to other areas or if adjustments must be made.
\end{description}





==> 5-Tola/sections/introduction.tex <==
\section{Introduction}


With the growing development in technology, the complexity of systems nowadays is increasing. More systems are operating in dynamic environments, where living creatures reside. If these systems fail, they may damage their surroundings, therefore they are called safety-critical systems~\cite{Knight02}.


It is crucial that such safety-critical systems operate in a safe manner. 
The increase of software in these types of systems makes the process of ensuring the system safety a challenge. This is due to the complications followed with the integration of software and systems engineering. A typical complication could be incomplete software specifications, where important details or requirements may be missing or stated incorrectly~\cite{Knight02}. 


%\textcolor{red}{Is this paragraph relevant?}
%An example of a safety-critical system, where the system requirements contained errors, is the Lufthansa Flight 2904\footnote{\url{https://en.wikipedia.org/wiki/Lufthansa_Flight_2904}}. The plane was attempting to land during stormy weather, where the braking functionality was switched off due to a safety feature. This resulted in the plane running off the edge of the runway and catching fire~\cite{Sommerville96}.


% Testing the physical system in every possible hazardous environment is difficult since some environments may depend on uncontrollable factors and the tests may be unethical. For example, an aircraft that must be able to fly during a thunderstorm is not physically tested while flying, but instead it is tested in controlled indoor labs~\cite{Moskvitch14}. 


Developing safety-critical systems is a complex process, where a large amount of time is spent on demonstrating the safety of the system, either by performing physical tests or formal verification~\cite{DSilva&08}. The effort required to develop safety-critical systems using traditional processes makes it hard to keep up with the shrinking time-to-market that is expected of such systems~\cite{Knight02}. Performing complete physical tests of a system to demonstrate its safety can be challenging due to the uncontrollable operating environments, such as changes in the surrounding atmosphere, and unethical tests, such as testing a pilot-controlled aircraft during a thunderstorm. Instead other Validation and Verification (V\&V) techniques must be used, such as simulation and co-simulation~\cite{Sun&09a,Helmut&17}. The focus of this paper is how co-simulation can be incorporated in the development process of safety-critical systems.


% A number of alternative techniques that have been suggested for the development and verification of safety-critical systems are: model-based systems engineering, simulation and co-simulation~\cite{Helmut&17,Knight02}. 


The rest of this paper starts with background information for the reader in Section~\ref{sec:background}. Afterwards, Section~\ref{sec:process_overview} gives a brief overview of the developed process, followed by Sections~\ref{sec:safety_analysis} and~\ref{sec:evidence_cosim} which go further into detail of the main steps of this process. Finally, Section~\ref{sec:conclusion} presents the concluding remarks and the potential future work.
% within the area of incorporating co-simulation in the development process of safety-critical systems.



